Improving the Tightness of Convex Relaxation Bounds for Training Certifiably Robust Classifiers

Convex relaxations are effective for training and certifying neural networks against norm-bounded adversarial attacks, but they leave a large gap between certifiable and empirical robustness. In principle, convex relaxation can provide tight bounds if the solution to the relaxed problem is feasible for the original non-convex problem. We propose two regularizers that can be used to train neural networks that yield tighter convex relaxation bounds for robustness. In all of our experiments, the proposed regularizers result in higher certified accuracy than non-regularized baselines.

==> include/dual.tex <==
% \subsection{The Dual View}
% Try to prove that the primal relaxation is indeed the best for this dual form?

==> include/experiments_828u.tex <==
\section{Experiments}
\subsection{Results with aforementioned methods}
Due to the limit of time, we have not get very complete results with the aforementioned method.
We have improved the certified error of a two-convolution network from 
0.5319 to 0.5239, but this approach is the most hopeful one we have tried.

\subsection{Another direction tried}
\begin{table}\label{tb:mnist}
\centering
\begin{tabular}{ c|c|c|c|c } 
 \hline
 Network & $\epsilon$ & Regularizer & Natural Err & Robust Err \\ 
 \hline
 2x400 FC  & 0.3 & No & 0.4360 & 0.1680 \\ 
2x400 FC  & 0.3 & Yes & 0.4263 & 0.1597 \\ 
LeNet  & 0.3 & No & 0.3230 & - \\ 
LeNet  & 0.3 & Yes & 0.3133 & 0.0787 \\ 
 \hline
\end{tabular}
 \caption{Comparing results with the convex relaxation approach~\citep{wong2018scaling} using the regularizer as given in Eq.~\ref{eq:ip_reg} on MNIST.}
\end{table}

\begin{table}\label{tb:cifar}
\centering
\begin{tabular}{ c|c|c|c|c } 
 \hline
 Network & $\epsilon$ & Regularizer & Natural Err & Robust Err \\ 
 \hline
 2 conv & 2 & No & 0.5319 & 0.3819 \\ 
2 conv  & 2 & Yes & 0.5213 & 0.3730\\ 
4 conv  & 2 & No & 0.4517 & 0.2925 \\ 
4 conv  & 2 & Yes & 0.4556 & 0.2929 \\ 
 \hline
\end{tabular}
 \caption{Comparing results with the convex relaxation approach~\citep{wong2018scaling} using the regularizer as given in Eq.~\ref{eq:ip_reg} on CIFAR10.}
\end{table}

We have tried a bunch of different things for this project.
Bearing the same spirit as the methods mentioned above, we have also tried another approach with the same goal.
Specifically, we want the optimality conditions of $c_t^\top x_L$ to match those of $c_{ij}^\top x_L$ in $\popt$. 
Consider $p=\infty$. 
To achieve the goal, we enforce the following regularizer while minimizing $p_{\ropt}^*$
\begin{equation}\label{eq:ip_reg}
    \sum_{j\in \cI_i, \delta^*_{ij}=0}|\langle(c_t^\top \cW_{L:1})_j, c_t^\top \cW_{i:1})_j \rangle|-\sum_{j\in \cI_i, \delta^*_{ij}>0}|\langle(\tanh(\alpha c_t^\top \cW_{L:1})_j), \tanh(\alpha c_t^\top \cW_{i:1})_j) \rangle|,
\end{equation}
where $\alpha>0$ is a hypter parameter and $\tanh$ is used to simulate the behavior of sign functions.
The first term trys to make $(c_t^\top \cW_{L:1})_j$ and $(c_t^\top \cW_{i:1})_j$ orthogonal, such that the optimal input perturbation $\delta_0^*$ will give rise to a zero $\delta_{ij}$ if propagated through $g_L$. 
The second term makes the signs of $(c_t^\top \cW_{L:1})_j$ and $(c_t^\top \cW_{i:1})_j$ to be either the same or contrary, such that the optimal perturbation gives a lower or upper bound in $g_L$. 
We tried this approach on both MNIST and CIFAR10. 
On CIFAR10, the input dimension is more than 3 times higher than MNIST, causing 3 times more memory usage. 
To make implement the experiments, we have adopted the projection approach as proposed by~\citep{wong2018scaling}, which projects $\cW_{i:1}$ with a Cauchy random matrix $R$ as $\cW_{i:1}R$, and estimate the $\ell_1$ norm (which is the dual norm of $\ell_\infty$ norm and used in $p_{\ropt}^*$) with $\text{median}(\cW_{i:1}R)$. 
Here by assuming the inner products of vectors are preserved under such a random projection, we use the inner products of $(c_t^\top \cW_{i:1}R)_j$ and $(c_t^\top \cW_{L:1}R)_j$ directly for the objective.
The results with random projection are given in Table~\ref{tb:mnist}
 and~\ref{tb:cifar}.

